Another Unsung Lowell Observatory Achievement: The First Infrared Observation of a Comet

Carl Lampland was the first to observe a comet in the infrared, a feat little known today because he failed to formally publish his data. I have retrieved the radiometry of this comet, C/1927 X1 (Skjellerup-Maristany), taken in broad daylight, from Lampland's logbook in the Lowell Observatory archives, and present a preliminary reduction of it here. There are similarities between Lampland's pioneering achievement and V. M. Slipher's discovery of the redshifts of the spiral nebulae (and thus, arguably, the expansion of the Universe). Each astronomer used state-of-the-art instrumentation, received rave reviews at American Astronomical Society meetings where their novel data were presented, and suffered under-recognition in ensuing decades. A common thread in these poor outcomes was their lackadaisical approach to formal publication - in Slipher's case, publishing in internal or secondary outlets, and in Lampland's case, not publishing at all.

==> PaxHeader/marcus20130129.tex <==
18 gid=1286109195
17 uid=533569006
20 ctime=1359492137
20 atime=1359492147
24 SCHILY.dev=234881026
22 SCHILY.ino=2595118
18 SCHILY.nlink=1

